InfluencerRank: Discovering Effective Influencers via Graph Convolutional Attentive Recurrent Neural Networks

As influencers play considerable roles in social media marketing, companies increase the budget for influencer marketing. Hiring effective influencers is crucial in social influencer marketing, but it is challenging to find the right influencers among hundreds of millions of social media users. In this paper, we propose InfluencerRank that ranks influencers by their effectiveness based on their posting behaviors and social relations over time. To represent the posting behaviors and social relations, the graph convolutional neural networks are applied to model influencers with heterogeneous networks during different historical periods. By learning the network structure with the embedded node features, InfluencerRank can derive informative representations for influencers at each period. An attentive recurrent neural network finally distinguishes highly effective influencers from other influencers by capturing the knowledge of the dynamics of influencer representations over time. Extensive experiments have been conducted on an Instagram dataset that consists of 18,397 influencers with their 2,952,075 posts published within 12 months. The experimental results demonstrate that InfluencerRank outperforms existing baseline methods. An in-depth analysis further reveals that all of our proposed features and model components are beneficial to discover effective influencers.

==> contents/analysis.tex <==
\section{Effective influencers vs. Noneffective influencers}\label{sec:characteristics}

We have 27,436 influencers in our dataset.
To compare characteristics of effective influencers and noneffective influencers, we divide the influencers into five groups.

(i) $IG_{tot}$: Total set of influencers contains 27,436 influencers.
(ii) $IG_{eff}$: Group of effective influencers whose effectiveness is greater than or equal to 1.0.
(iii) $IG_{non}$: Group of noneffective influencers whose effectiveness is less than 1.0.
(iv) $IG_{top}$: Top 10 percentile of effective influencers
(v) $IG_{bot}$: Bottom 10 percentile of influencers


\paragraph{Topics of influencers}
%Topic
\begin{figure}
\centering
\includegraphics[width=8cm]{figures/char_topic.pdf}
\caption{Topics of influencers in each group.}
\label{fig:char_topic}
\end{figure}

The fashion, travel, and pet influencers tend to be more effective than the beauty, food, and interior influencers.


\paragraph{Other features}

\begin{figure}
\centering
\includegraphics[width=8cm]{figures/char_features.pdf}
\caption{Characteristics of influencer groups}
\label{fig:char_features}
\end{figure}


